Understanding Binary Systems -- a Comparison between COSMIC and MESA

We compare the evolution of binary systems evolved in the MESA stellar evolution code to those in the COSMIC population synthesis code. Our aim is to convey the robustness of the equations that model binary evolution in the COSMIC code, particularly for the cases of high mass stars with closely orbiting compact object companions. Our larger goal is to accurately model the rates of these systems, as they are promising candidates for the progenitor systems behind energetic, longer lasting, radio bright GRB jets. These systems also may be key contributors to the rates of binary black hole mergers throughout our universe.

==> Makefile <==
LATEXMK=latexmk

SRC=header.tex \
    main.bib 

default: bhns

all: bhns

bhns: main.pdf

%.pdf: %.tex ${SRC} $(shell find figures/)
	${LATEXMK} -f -pdf $<

clean:
	rm -f ./*.aux ./*.bbl ./*.blg ./*.log ./*.nav ./*.out ./*.snm ./*.toc ./*.fls ./*.fdb_latexmk mainNotes.bib main.pdf



==> figurecalls.tex <==
%\begin{figure*}[htp]
%    \centering
%    \includegraphics[width=0.5\textwidth,height=0.3\textheight]{cosmic_figures/porb=1.5 sep(fixedax).png}\includegraphics[width=0.5\textwidth, height=0.3\textheight]{mesa_figures/separation_1.5days.png}
 %   \caption{Separation of primaries at 1.5 day orbital period - COSMIC on the left and MESA on the right.}
 %   \label{fig:gaussfit}
%\end{figure*}

%MESA FIGURE:
% \begin{figure*}[htp]
%    \centering
%    \includegraphics[width=15cm]{mesa_figures/separation_1.5days.png}
%   \caption{MESA figure for $M_{*}=25M_{\odot}$, BH=$15M_{\odot}$ of orbital period 1.5 days. Initially looks very similar, but when MESA runs into ROLF, the separation explodes.}
%    \label{fig:mesa_aorb1.5days}
%\end{figure*}
%\begin{figure*}[htp]
%    \centering
 %   \includegraphics[width=15cm]{mesa_figures/separation_1.5days_initorbitsync.png}
%    \caption{MESA figure for $M_{*}=25M_{\odot}$, BH=$15M_{\odot}$ same as figure 2 but with the flag initial\_orbit\_sync.}
%    \label{fig:mesa_aorb1.5days_sync}
%\end{figure*}
%MESA ENDS
%\begin{figure}
 %   \centering
 %   \includegraphics[width=0.5\textwidth,height=0.3\textheight]{cosmic_figures/porb=3.0 sep (fixedax).png}\includegraphics[width=0.5\textwidth, height=0.3\textheight]{mesa_figures/separation_3.0days.png}
%    \caption{Separation of primaries at 3 day orbital period - COSMIC on the left and MESA on the right.}
%    \label{fig:3.0sep}
%\end{figure}
%MESA FIGURES:
%\begin{figure*}[htp]
%    \centering
%    \includegraphics[width=15cm]{mesa_figures/separation_3.0days.png}
%    \caption{MESA figure for $M_{*}=25M_{\odot}$, BH=$15M_{\odot}$ of orbital period of 3 days.}
%    \label{fig:mesa_aorb3.0days}
%\end{figure*}
%\begin{figure*}[htp]
%    \centering
%    \includegraphics[width=15cm]{mesa_figures/separation_3.0days_initorbitsync.png}
 %   \caption{MESA figure for $M_{*}=25M_{\odot}$, BH=$15M_{\odot}$ of orbital %period of 3 days with the initial\_orbit\_sync.}
%    \label{fig:mesa_aorb3.0days_sync}
%\end{figure*}
%END MESA FIGURES


%\begin{figure}
 %   \centering
 %   \includegraphics[width=0.5\textwidth,height=0.3\textheight]{cosmic_figures/porb=1.5 AM(2).png}\includegraphics[width=0.5\textwidth, height=0.3\textheight]{mesa_figures/Jspin_1.5days.png}
  %  \caption{Spin of primaries at 1.5 day orbital period - COSMIC on the left and MESA on the right.}
 %   \label{fig:1.5spin}
%\end{figure}

%MESA FIGURE BEGINS
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{mesa_figures/Jspin_1.5days.png}
    \caption{MESA figure of spin angular momentum for $M_{*}=25M_{\odot}$, BH=$15M_{\odot}$ of orbital period of 1.5 days.}
    \label{fig:mesa_jspin1.5days}
\end{figure*}
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{mesa_figures/Jspin_1.5days_initorbitsync.png}
    \caption{MESA figure of spin angular momentum for $M_{*}=25M_{\odot}$, BH=$15M_{\odot}$ of orbital period of 1.5 days with initial\_orbit\_sync.}
    \label{fig:mesa_jspin1.5days_sync}
\end{figure*}
%MESA FIGURE ENDS



\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth,height=0.3\textheight]{cosmic_figures/porb=3.0 AM(2).png}\includegraphics[width=0.5\textwidth, height=0.3\textheight]{mesa_figures/Jspin_3.0days.png}
    \caption{Spin of primaries at 3.0 day orbital period - COSMIC on the left and MESA on the right.}
    \label{fig:3.0spin}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=15cm]{cosmic + mesa figures/COSMIC:MESA - Jspin (3.0).png}
    \caption{COSMIC and Mesa comparison of spin of primaries at 3.0 day orbital period.}
    \label{fig:COSMIC/MESA_3.0spin}
\end{figure}
%MESA FIGURE BEGINS
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{mesa_figures/Jspin_3.0days.png}
    \caption{MESA figure of spin angular momentum for $M_{*}=25M_{\odot}$, BH=$15M_{\odot}$ of orbital period of 3.0 days.}
    \label{fig:mesa_jspin3.0days}
\end{figure*}
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{mesa_figures/Jspin_3.0days_initorbitsync.png}
    \caption{MESA figure of spin angular momentum for $M_{*}=25M_{\odot}$, BH=$15M_{\odot}$ of orbital period of 3 days with initial\_orbit\_sync.}
    \label{fig:mesa_jspin3.0days_sync}
\end{figure*}
%MESA FIGURE ENDS
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{cosmic + mesa figures/COSMIC:MESA - Jspin (1.5).png}
    \caption{COSMIC and Mesa comparison of spin of primaries at $M_{*}=25M_{\odot}$ with a black hole companion at $20M_{\odot}$, and $15M_{\odot}$ with a 1.5 day orbital period.}
    \label{fig:cosmic/mesaFig6}
\end{figure*}
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{cosmic + mesa figures/COSMIC:MESA - Sep (1.5).png}
    \caption{COSMIC and Mesa comparison of separation of primaries at $M_{*}=25M_{\odot}$ with a black hole companion at $20M_{\odot}$, and $15M_{\odot}$ with a 1.5 day orbital period.}
    \label{fig:cosmicFig}
\end{figure*}
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{cosmic + mesa figures/COSMIC:MESA - Sep (3.0).png}
    \caption{COSMIC and Mesa comparison of separation of primaries at $M_{*}=25M_{\odot}$ with a black hole companion at $20M_{\odot}$, and $15M_{\odot}$ with a 3 day orbital period.}
    \label{fig:cosmicFig4}
\end{figure*}
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{cosmic_figures/Sep(3); porb=3.0.png}
    \caption{COSMIC figure of separation of primaries at $M_{*}=25M_{\odot}$ with a black hole companion at $20M_{\odot}$, $15M_{\odot}$, and $5M_{\odot}$ with a 3 day orbital period.}
    \label{fig:COSMIC/MESAFig1}
\end{figure*}
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{cosmic_figures/Spin(3); porb=3.0.png}
    \caption{COSMIC figure of spin of primaries at $M_{*}=25M_{\odot}$ with a black hole companion at $20M_{\odot}$, $15M_{\odot}$, and $5M_{\odot}$ with a 3 day orbital period.}
    \label{fig:COSMICFig2}
\end{figure*}
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{cosmic_figures/Sep(3);porb=1.5.png}
    \caption{COSMIC figure of separation of primaries at $M_{*}=25M_{\odot}$ with a black hole companion at $20M_{\odot}$, $15M_{\odot}$, and $5M_{\odot}$ with a 1.5 day orbital period.}
    \label{fig:COSMICFig3}
\end{figure*}
\begin{figure*}[htp]
    \centering
    \includegraphics[width=15cm]{cosmic_figures/Mass(3); porb=1.5.png}
    \caption{COSMIC figure of mass of primaries at $M_{*}=25M_{\odot}$ with a black hole companion at $20M_{\odot}$, $15M_{\odot}$, and $5M_{\odot}$ with a 1.5 day orbital period.}
    \label{fig:COSMICFig4}
\end{figure*}
